Entity-Specific Sentiment Classification of Yahoo News Comments

Sentiment classification is widely used for product reviews and in online social media such as forums, Twitter, and blogs. However, the problem of classifying the sentiment of user comments on news sites has not been addressed yet. News sites cover a wide range of domains including politics, sports, technology, and entertainment, in contrast to other online social sites such as forums and review sites, which are specific to a particular domain. A user associated with a news site is likely to post comments on diverse topics (e.g., politics, smartphones, and sports) or diverse entities (e.g., Obama, iPhone, or Google). Classifying the sentiment of users tied to various entities may help obtain a holistic view of their personality, which could be useful in applications such as online advertising, content personalization, and political campaign planning. In this paper, we formulate the problem of entity-specific sentiment classification of comments posted on news articles in Yahoo News and propose novel features that are specific to news comments. Experimental results show that our models outperform state-of-the-art baselines.

==> Files/algo-2.tex <==
\begin{algorithm}
%\begin{small}
\centering
\begin{algorithmic}[1]

\Function {$\tt extractLocalContext$}{$s,e_1,e_2$}
	\State $l_1 \gets \phi$ and $l_2 \gets \phi$; {\color{light-gray}{\scriptsize{// $l_1$ and $l_2$ are local contexts of $e_1$ and $e_2$, respectively.}}}
	\State $D \gets {\tt getDependencyTree}(s)$;
	\If{$s:=cl_1$ but $cl_2$ $\&\&$ $e_1 \in cl_{1/2}, e_2 \in cl_{2/1}$} {\color{light-gray}{\scriptsize{// if $s$ contains two clauses $cl_1$ and $cl_2$ connected by ``but'', and $e_1$ belongs to either one clause and $e_2$ belongs to the other clause}}}
		\State $l_1 \gets cl_{1/2}$, $l_2 \gets cl_{2/1}$;
	%\If {$e_1$ and $e_2$ occur in clauses connected by ``but''}
	%		\State \Return $cl_1$, $cl_2$
	%		\Comment{$cl_1$, $cl_2$ are the clauses having $e_1$ and $e_2$ resp.}
	
	
	%\If {$e_1$ and $e_2$ occur in clauses connected by ``but''}
	%		\State \Return $cl_1$, $cl_2$
	%		\Comment{$cl_1$, $cl_2$ are the clauses having $e_1$ and $e_2$ resp.}
	\ElsIf{$e_1$ and $e_2$ are compared in $s$} {\color{light-gray}{\scriptsize{// if $s$ is a comparative sentence, and $e_1$ and $e_2$ are compared in $s$}}}
			\State $[p_1,p_2] \gets split(comparative\_term,s)$; {\color{light-gray}{\scriptsize{// split $s$ on the comparative term and store the substrings in $p_1$ and $p_2$.}}}
			%\State Split $s$ at the comparative and add the comparative to the left part.
			\State $l_1 \gets p_1 \cup comparative\_term$, $l_2 \gets p_2$; {\color{light-gray}{\scriptsize{// $p_1$, $p_2$ are the substrings containing $e_1$ and $e_2$, respectively.}}}
			%\Comment{$p_1$, $p_2$ are the parts having $e_1$ and $e_2$ resp.}
	\Else	 \mbox{	}	{\color{light-gray}{\scriptsize{// in all other cases of constructs of $s$}}}
			\State $l_1 \gets$ ($\pm 3$ tokens around $e_1$ in $s$) $\cup$ (children and parent of $e_1$ in $D$);
			\State $l_2 \gets$ ($\pm 3$ tokens around $e_2$ in $s$) $\cup$ (children and parent of $e_2$ in $D$);
			%\State \Return $l_1, l_2$
	\EndIf
	\State \Return $l_1, l_2$.
\EndFunction
%\State \textbf{\textit Output}: $c_1$, $c_2$
%\State \textbf{\textit Output}: Classifiers $C_I$, $C_D$.
\end{algorithmic}
%\end{small}
\caption{Local Context Extraction Algorithm}
\label{contextExtraction2}
\end{algorithm}


==> Files/algo.tex <==
\begin{algorithm}[!ht]
\caption{Context Extraction Algorithm}
\label{contextExtraction1}
\begin{algorithmic}[1]
\State \textbf{Input}: news comment $C$; entities $e_1$, $e_2$; sets of pronouns $P$:\{his, her, herself, him, himself, he, she\}, $NP$:\{it, their, them, they\}. 
\State \textbf{Output}: contexts $c_1$ and $c_2$ of $e_1$ and $e_2$, respectively.
\State $c_1 \gets \phi$ and $c_2 \gets \phi$;
\If{$e_1$ is null}
		\State $c_2 \gets C$; {\color{light-gray}{\scriptsize{// $C$ becomes the context of $e_2$.}}}
\ElsIf{$e_2$ is null}
		\State $c_1 \gets C$; {\color{light-gray}{\scriptsize{// $C$ becomes the context of $e_1$.}}}
\ElsIf{$e_1$ and $e_2$ are connected with ``and'' or ``,''}
		%\State Merge $e_1$ and $e_2$;
		\State $c_1 \gets C$, $c_2 \gets C$;  {\color{light-gray}{\scriptsize{// $C$ becomes the context of  $e_1$ and $e_2$, i.e., entities separated by ``and'' or ``,'' have the same sentiment.}}}
\Else
		\State $S \gets split(.|?|!,C)$; {\color{light-gray}{\scriptsize{// find sentences in $C$.}}}
		%\State $(c_1,c_2) \gets getContext()$	
		\ForAll {$s \in S$}
        		\If{$e_1 \, =\!\mytilde \, s \,$ $\&\&$ $\, e_2 \, = \!\mytilde \, s$}
		{\color{light-gray}{\scriptsize{// if both $e_1$ and $e_2$ are present in $s$, get local contexts, and add them to $c_1$ and $c_2$.}}}
								\State $(l_1,l_2) \gets {\tt {extractLocalContext}}(s,e_1,e_2)$;
								\State $c_1 \gets c_1 \cup l_1$ and $c_2 \gets c_2 \cup l_2$;
						\ElsIf{$e_1 \, =\!\mytilde \, s$} {\color{light-gray}{\scriptsize{// if only $e_1$ is present in $s$, add $s$ to $c_1$.}}}
								\State $c_1 \gets c_1 \cup s$;
						\ElsIf{$e_2 \, =\!\mytilde \, s$} {\color{light-gray}{\scriptsize{// if only $e_2$ is present in $s$, add $s$ to $c_2$.}}}
								\State $c_2 \gets c_2 \cup s$;
						\Else  \mbox{	}%{$s \, !\mytilde  \, e_1  \, \&\&  \, s\, !\mytilde e_2$}
						{\color{light-gray}{\scriptsize{// if none of $e_1$ or $e_2$ is present in $s$}}}
								\If{$P$ \, !\mytilde  \, $s$} {\color{light-gray}{\scriptsize{// if no  mentions from $P$ are in $s$, regardless of mentions from $NP$, add $s$ to both $c_1$ and $c_2$.}}}
										\State $c_1 \gets c_1 \cup s$ and $c_2 \gets c_2 \cup s$;
								\ElsIf{$P \, =\!\mytilde \, s  \,$ $\&\&$  $\, NP !\mytilde  \, s$} {\color{light-gray}{\scriptsize{// if mentions from $P$ are present in $s$, but no mentions from $NP$}}}
										\If{$e_1 :=PER \&\& e_2 := PER$} {\color{light-gray}{\scriptsize{// if both $e_1$ and $e_2$ are person entity type, add $s$ to both $c_1$ and $c_2$.}}}
												\State  $c_1 \gets c_1 \cup s$ and $c_2 \gets c_2 \cup s$;
										\ElsIf{$e_1 := PER$ }  {\color{light-gray}{\scriptsize{// if only $e_1$ is person entity type, add $s$ to $c_1$.}}}
												\State $c_1 \gets c_1 \cup s$;
										\ElsIf{$e_2 := PER$}  {\color{light-gray}{\scriptsize{// if only $e_2$ is person entity type, add $s$ to $c_2$.}}}
												\State $c_2 \gets c_2 \cup s$;
										\EndIf
								\Else \mbox{	} {\color{light-gray}{\scriptsize{// in all other cases, add $s$ to both $c_1$ and $c_2$.}}}
										\State $c_1 \gets c_1 \cup s$ and $c_2 \gets c_2 \cup s$;
								\EndIf						
						\EndIf
				\EndFor	
\EndIf
%\Function {$getContext$}{$e_1$, $e_2$, $C$, $N$, $NP$, $S$}
\State \Return $c_1,c_2$
%\EndFunction
\end{algorithmic}
\end{algorithm}


==> Files/annotation.tex <==
\begin{table}[ht]
\begin{centering}
%\begin{footnotesize}
%\begin{small}
%\begin{center}
	\begin{tabular}{@{}l p{4.00 in}@{}}
	%\begin{small}
	\toprule
	\textbf{Feature Name} & \textbf{Description}\\
	Total comments&$41,852,453$\\
	No. of conversations&$9,586,835$\\
	No. of reply comments&$21,830,249$\\
	No. of isolated comments&$10,435,369$\\
	No. of users&$$\\
	\bottomrule
	\end{tabular}
	%\end{footnotesize}
	%\end{small}
	\caption{Data description.}
	\label{annoData}		
%end{small}
%\end{scriptsize}
\end{centering}
\end{table}

==> Files/approach_copy.tex <==
\section{Problem Characterization}
\label{approach}
%In this section, we first state our problem and then describe the proposed approach.
%\subsection{Problem Characterization}

Sentiment analysis, or opinion mining, has been actively researched in the domain of online review sites aiming at summarizing user opinions about different products. This problem faces many challenges such as dealing with unstructured text and noisy user input, and mapping sentiment to objects or entities \cite{LiuSurvey}. Beyond these, the problem of opinion mining of news comments brings additional challenges, including: a large variety of domains (e.g., politics, sports, technology, and entertainment), lack of use of important sentiment clues (e.g., no use of emoticons), and the use of rhetorical questions. These additional, less studied challenges give rise to the unique design of our model. % (as will be described in the next section). 

The main tasks of opinion mining of news comments are: (1) extracting entities from news comments, and (2) identifying users' sentiments about the extracted entities. Although both tasks have their own particular challenges, the second task is central to our study. Note that to extract entities from news comments, we used a Named Entity Recognizer (NER) developed internally at {\em Yahoo} that we refer to as YNER here. In experiments, we compared the performance of three NER libraries: Stanford NER, Perl NER library, and YNER, and found that YNER was the most effective. It typically identifies three types of entities in a piece of text: person, place, and organization. The problem that we address in this paper can be formulated as follows:

{\bf Problem Formulation:} Given a comment and an entity, classify the sentiment expressed in the comment about that particular entity into one of the three sentiment classes: positive (denoted by $+1$), negative (denoted by $-1$) or neutral (denoted by $0$). 

To address this problem, we decompose it into two parts. We first link the target entity with its sentiment context. Specifically, when multiple entities are present in a comment, each entity must be linked to its own context, i.e., the words/phrases in the comment that are related to the entity. This is necessary to identify the context for each entity since entities in a comment may have different sentiments or some entities may not even have any sentiment at all associated with them (as illustrated in the examples below).

{\bf Example 6:} {\em ``Let me get this straight.} {Hillary Clinton} {\em saved us \$100 million dollars, but, how does that compare to the 4 trillion the} {Obama} {\em administration has spent?''}

In this example, the sentiment is positive for Hillary Clinton, but negative for Obama. 
 
{\bf Example 7:} {\em In Ohio, voting for} Romney {\em who said he would let} GM \& Chrysler {\em go bankrupt is like  paying a guy to rebuild your house that he burned down.}

Here, the sentiment is negative for Romney. However, GM and Chrysler, identified as entities by YNER, do not have any sentiment associated with them,
% and in particular, CNN is irrelevant with respect to the commenter's opinion. 


%We want to extract entities that are mentioned in a comment and identify sentiments expressed about those entities. So, the problem can be divided into two sub parts: 
%\begin{itemize}
%\item {\bf Extract entities in comments}: 
%\item {\bf Identify sentiments about extracted entities}: This is essentially the main problem we will address in this work. It can be further decomposed into two parts: 
%	\begin{enumerate}
%		\item {\bf Link entity with its sentiment context}: When there are multiple entities present in a comment, each entity must be linked to its context, i.e., the words/phrases in the comment that are linked to it. This is required as the entities in a comment may have different sentiments or some entities may not have any sentiment (in case of irrelevant entities (as discussed in Section~\ref{intro})).
%		\item {\bf Identify sentiment of the context}: We identify three sentiments for an entity: positive, negative or neutral. 
%	\end{enumerate}
%\end{itemize}

%Based on the above discussion, we now state our problem: {\bf {\em }}. 

Second, after entities are linked to their contexts, we identify the sentiment for an entity to be positive, negative or neutral, based on the sentiment of its context. In the rest of the paper, we will use the term entity and its context interchangeably while referring to the sentiment of the entity. For example, saying that an {\em entity is polar} is equivalent to saying that the {\em entity has a polar context.}

\input{Files/algo.tex}

\subsection{Extracting the Context for an Entity}
The context of an entity contains the words, phrases and sentences that refer to the entity. We used several heuristics to extract the context of an entity. When there is a single entity in a comment, then the entire comment is considered as the context of the entity. If a comment contains multiple entities, we segment the comment into multiple contexts, one for each entity. The reason for this is that different sentiments could be expressed about the different entities in the comment (as shown in the {\bf Examples 1} and {\bf 2}). We use several rules and natural language processing (NLP) resources to extract contexts for entities.  More precisely, we use the Stanford NLP toolkit's PCFG parser to obtain the dependency tree and part-of-speech tags. Algorithm~\ref{contextExtraction1} explains the process of extracting contexts when there are two entities present in a comment. For simplicity, we show this context-extraction algorithm for the two entity case only, but it can easily be extended to cases where more than two entities are present in a comment.

The algorithm takes as input: a news comment $C$, entities $e_1$, $e_2$ present in the comment, a set of third person singular pronouns, $P$: \{his, her, him, he, she\} and a set containing three pronouns, $NP$: \{it, their, them\}. The output of the algorithm is the pair of contexts $c_1$ and $c_2$ corresponding to $e_1$ and $e_2$, respectively. Initially, $c_1$ and $c_2$ are set to be empty (line 3). 
%The function $\tt getSentence$ returns an array ($S$) of all the sentences in $C$ by splitting $C$ on full stop, question mark and exclamation mark (lines 4 and 42-44). 
The algorithm first checks if one of the two entities, either $e_1$ or $e_2$, is null, and if so,  returns the entire comment as the context for the non-null entity (lines 4-7). If $e_1$ and $e_2$ are both non-null, and if they are connected by ``and'' or ``,'', the entire comment becomes the context for both entities (lines 8,9). The reason for this is that it is highly likely that both entities will have the same sentiment (see the example below in which the sentiment for both Obama and Romney is negative).  

{\bf Example 8:} {\em Both} Obama {\em and} Romney {\em are surrounded by Wall Street and Federal Reserve Criminals.}

This rule is very helpful when there are many entities in a comment and most of them are connected with AND or ``,''. In the following example, Yahoo, ABC, NBC, MSNBC, CNN and CBS are connected by ``,''and all have negative sentiment. Following this rule, we treat this comment as a single-entity comment and hence do not segment it into contexts of the $6$ entities in it.

{\bf Example 9:} {\em Breaking News...}Yahoo, ABC, NBC, MSNBC, CNN, CBS {\em flunk on telling the truth about anything 99\% of the time..}


\input{Files/algo-2.tex}

If $e_1$ and $e_2$ are not connected by ``and'' or ``,'', first all sentences in $C$ are generated by splitting $C$ on full stop, question mark, and exclamation mark and they are stored in $S$ (line 11). Then, the algorithm checks for the presence (using $=\mytilde$ operator) or absence (using $!\mytilde$ operator) of $e_1$, $e_2$ and the pronouns in $P$ and $NP$ in each sentence $s \in S$. If a sentence $s$ contains explicit mentions of both the entities (line 13), then the $\tt getLocalContext$ subroutine is called to extract the local context of each entity from $s$ (line 14) (see Algorithm \ref{contextExtraction2}).
%We will discuss this function later. 
If only one entity is present in $s$, then $s$ is added to its current context (lines 16-19). Further, if none of the entities appear in $s$, then the algorithm checks for the presence of $P$ and $NP$ pronouns and the entity type (person or non-person) of $e_1$ and $e_2$ (lines 21-33). The reason for this is that $P$ pronouns can only be used to refer to a person entity, whereas $NP$ pronouns can be used to refer to both person and non-person entities. If $s$ does not contain explicit mentions of any of the two entities and it either does not have $P$ pronouns or it has both $P$ and $NP$ pronouns, then $s$ is added to the context of both the entities (lines 20-22, 32). If $s$ has $P$ pronouns and does not contain $NP$ pronouns, then it is added to the person entity (lines 23-30). 



If $s$ contains both $e_1$ and $e_2$, then the function that extracts the local context for each entity, $\tt extractLocalContext$ is called (line 14). The pseudocode is shown in Algorithm \ref{contextExtraction2}. $\tt getDependencyTree(s)$ is used to get the dependency tree $D$ of $s$. We used the Stanford PCFG parser that has typed dependency representation to get the dependency tree~\cite{de2006generating}. If $e_1$ and $e_2$ occur in clauses that are connected with ``but'' in $s$ (each clause has either $e_1$ or $e_2$), then the respective clauses are returned as local contexts for the entities (lines 4,5). If $s$ contains a comparison between $e_1$ and $e_2$, then it is split at the comparative term (adjective or adverb), with the comparative term added to the left part, and the two parts are returned as local contexts (lines 6-8). If the sentence does not satisfy the ``but'' and the comparison conditions, then we use a window of $\pm3$ tokens around each entity and their parent and children in $D$ as their respective local contexts $(l_1,l_2)$ (lines 9-11). If there are less than $3$ words between $e_1$ and $e_2$, then we add all the words that are in between to the context of both the entities. Similarly, if $e_1$ and/or $e_2$ have less than $3$ tokens on any of their sides then we add all the words on the side that has less than $3$ tokens to the context. Other previous works have used a window of $\pm3$ tokens as the context for entities~\cite{cit}. We found that this heuristic fails in capturing the long tail dependencies, and hence, we also added the parent and children of entities in the dependency tree to their context. In cases 
%% give example


%\input{Files/featureTable.tex}

\subsection{Identifying the Sentiment of Contexts}
After obtaining the contexts of entities, we classify their sentiment into {\em positive}, {\em negative} or {\em neutral} sentiment classes. We model the task of identifying sentiment as two step classification. In the first step, we classify the context of an entity into {\em polar} versus {\em neutral} sentiment classes. Next, we classify the polar entities into {\em positive} or {\em negative} sentiment classes. In the next subsections, we describe various features used in our classification models and our reasoning behind using them. We first discuss the features used for the neutral vs. polar classification model, and then discuss the features used for positive vs. negative classification model. % (see Figure \ref{features} for a list of these features). %Figure \ref{features} lists and defines the various features used in our classification model. Specifically, we extract the following features from the news comments.

\subsubsection{Neutral vs. Polar Classification}
As already discussed, comments posted on news sites contain entities that are irrelevant with respect to sentiment analysis. {\bf Example 2} in Section 3 shows an example of an irrelevant entity. These entities have no sentiment associated with them and have to be filtered out before conducting sentiment analysis of the comments. We address this problem by classifying entities as polar or neutral. Irrelevant entities are classified as neutral. Generally, content features and lexicon features form the basis of polar versus neutral classification. However, in our data, we find some other interesting properties (specific to entities) that can be very helpful in identifying neutral and polar entities. For example, an entity that is a subject or direct object (of the subject) in a comment is more likely to be polar than an entity that is a prepositional object. Also, an entity of {\em person} type is more likely to be polar than an entity that is of {\em non-person} type. Let us consider the following example.

{\bf Example 10:} Bush {\em didn't blame anyone for trashing the White House, the 2001 recession, or for the 3 major attacks} on America.

{\bf Example 11:} Obama {\em stole 716 billion dollars we paid} into medicare {\em to save his} bummercare.

%1. ``{\em Bush} didn't blame anyone for trashing the white house, the 2001 recession, or for the 3 major attacks {\em on America}.
%2. ``{\em Obama} stole 716 billion dollars we paid {\em into medicare} to save his {\em bummercare}.''

In {\bf Example 10}, {Bush} is the subject, whereas {America} is the prepositional object. In {\bf Example 11}, {Obama} is the subject, {medicare} is the prepositional object and {bummercare} is the direct object. As can be seen, Obama and Bush are polar entities, whereas America and medicare are neutral entities.


Based on this reasoning, we extract the following features for all entities in a comment:
\begin{itemize}
	\item {\bf IsPerson:} If the entity is of {\em person} type (1 if yes, 0 otherwise). To compute this feature, we look at the entity type output by YNER.
	\item {\bf IsSubjObj:} If the entity is the subject, direct object, prepositional object or none of the three. (3 if subject, 2 if direct object, 1 if prepositional object, 0 otherwise). To compute this feature, we check if the entity has the following dependencies in the dependency tree: {\em nsubj} (nominal subject), {\em dobj} (direct object) and {\em pobj} (prepositional object).
	\item {\bf HasPolarityClues:} If there are any polarity clues in the context of the entity (1 if yes, 0 otherwise). 
	\item {\bf SentiPos:} This feature is calculated from the positive sentiment score given by the SentiStrength algorithm~\cite{thelwall2012sentiment} (0 if the score is 1, 1 otherwise) (we explain the scores output by SentiStrength in Section~\ref{polarityClassification}).
	\item {\bf SentiNeg:} This feature is calculated from the negative score given by the SentiStrength algorithm~\cite{thelwall2012sentiment} (0 if the score is -1, -1 otherwise) 
 %	\item {\bf SentiPosNeg:} Ratio of positive and negative scores given by the SentiStrength algorithm \cite{sentistr}.
\end{itemize}
Apart from the above features, we use the following two high precision rules to detect neutral and polar entities.

{\bf Rule 1: IsVerb: } If an entity is used as a verb, then it is {\em neutral}. Entities such as  Google, Bing, and Youtube, can be used as a verb and have neutral sentiment in those cases. Let us consider the following example. 

{\bf Example 12:} Marci Alt {\em is an arsonist.} Google {\em her name and see the mugshot of this man like plaid wearing lesbian.}

Here, the comment has a negative sentiment for the entity Marci Alt and neutral sentiment for Google. An entity satisfies this rule if it is used only as a verb in the entire comment.

{\bf Rule 2: HasAMod: } If an entity is modified by an adjective, then it is polar. We look for the {\em amod(entity, adjective)} dependency in the dependency tree to check if an entity satisfies the rule. Some of the example phrases are {\em {\bf conservative} FOX}, {\em {\bf stupid} democrats}, etc.
%\begin{itemize}
%	\item {\bf IsVerb}: If an entity is used as a verb then it is {\em neutral}. Entities like Google, Bing, Youtube, etc can be used as a verb and have neutral sentiment in those cases. Let us consider this example. "Marci Alt is an arsonist. Google her name and see the mugshot of this man like plaid wearing lesbian.` Here, the comment has a negative sentiment for the entity {\em Marci Alt} and neutral sentiment for Google. An entity satisfies this rule if it is used only as a verb in the entire comment.
%	\item {\bf IsAmod}: If an entity is modified by an adjective then it is polar. We look for the {\em amod(entity, adjective)} dependency in the dependency tree to check if an entity satisfies the rule. Some of the example phrases are {\em {\bf conservative} FOX}, {\em {\bf stupid} democrats}, etc.
%\end{itemize}
\subsubsection{Positive vs. Negative Classification}
\label{polarityClassification}
After obtaining the polar entities, we classify the sentiment about those entities into positive or negative sentiment classes. We use the following features for the polarity classification, which are summarized in Table~\ref{features}.

\begin{figure}[t]
\centering
{\includegraphics[scale=0.36]{Files/table1.png}}
\caption{\label{features}Description of various features extracted from the context of an entity for polarity classification.} 
\end{figure}

%\begin{enumerate}[(a)]
{\bf (a) Polarity Clues:}
Polarity clues are the words, phrases, or symbols used to express polarity of opinions/emotions in speech or written text. Polarity clues have been used extensively by the previous works on sentiment analysis~\cite{sentiWords, unsup1}. We use two lexicons for getting polarity clues: subjectivity lexicon from MPQA corpus developed by Weibe et al.~\cite{mpqa} and polarity lexicon developed by Hu et al.~\cite{lexicon}. The subjectivity lexicon contains subjectivity clues with prior polarity positive, negative or neutral. The second lexicon is adapted from the subjectivity lexicon, but it does not contain neutral subjectivity clues. As we will describe later, neutral subjectivity clues, if connected with negation words, become negative in polarity. Thus, we take the neutral clues from the first lexicon and polar clues from the second lexicon. In addition, we added some words (e.g., arsonist and guts) to both the lexicons. We believe that such words will appear in other domains that involve user generated data. Finally, we got $2006$ positive clues, $4713$ negative clues and $572$ neutral subjectivity clues. We extract three features { NumPos}, { NumNeg}, and { PosVsNeg} from the context of an entity. { NumPos} and { NumNeg} are the number of positive and negative polarity clues in the context, respectively. { PosVsNeg} is the number of positive polarity clues over negative polarity clues and is calculated by dividing { NumPos}+1 by { NumNeg}+1. 

We use the following rules to count the number of polarity clues:

{\em Rule 1: Negation: } In general, the presence of negation words reverses the polarity of the sentiment expressed by a polarity clue. Example of negation words are no, not, never, do not, etc. If a polarity clue is connected to a negation word then we reverse its polarity. We say a polarity clue and a negation word are connected if they co-occur in a window of $3$ tokens. If a neutral subjectivity clue is connected to a negation word, then its polarity is taken as negative. For example, {\em believe} is a subjectivity clue with prior polarity neutral but if used with a negation (e.g. I do not believe or I cannot believe) expresses negative sentiment. We use a list of $50$ negation words.

{\em Rule 2: Quotes:} Users often put polarity clues in quotes or in a quoted phrase to mean entirely opposite sentiment as compared to the sentiment expressed by the clue. Let us consider this example. 

{\bf Example 13:} The Republican party {\em also faces a steep climb with the "sane people" demographic.}

Here, the clue {\em sane} is in a quoted phrase {\em sane people}. Prior polarity of {\em sane} is positive. However, in this case, it is used to express negative sentiment about the Republican party. If a polarity clue is in a quoted phrase then we reverse its polarity.



{\em Rule 3: ``but'' rule:} Usually, sentiment expressed in clauses connected with ``but'' have opposite polarities. We take into account this property, while aggregating polarity clues for the entities. If clauses containing two entities are connected with ``but'' and there are explicit polarity clues in the context only one of the entities, then we increase the count of the clue of opposite polarity for the other entity. % give an example here.

{\bf Example 14:} {\em Read how} Bush {\em tried to control the financial situation with new regulations} {\bf but} {\em democrats  blocked him. Democrats are pathetic, greedy liars. Democrats want poverty and racism to continue, otherwise they will lose their power.}

Here, Bush and democrats occur in clauses connected with BUT and have opposite sentiment. For democrats, there are explicit negative clues (pathetic, greedy) but we do not have explicit polarity clues for Bush. In this case, we take the value of $NumPos$ feature for Bush as $1$.

{\em Rule 4: Comparatives:} If two entities are present in a comparative clause and one of the entities does not have explicit polarity clue (in its context), then for that entity we increment the number of opposite polarity clue. We identify two most common types of comparatives: adjectival comparatives and adverbial comparatives (Refer to the paper by Jindal et al.~\cite{comparative} for detailed discussion on comparative sentences). We look for {\em JJR} and {\em RBR} part-of-speech tags between entities to identify comparative adjectives and comparative adverbs, respectively. Let us consider this example. 

{\bf Example 15:} {\em The} samsung {\em galaxys' are way better than all the mobile products} apple {\em puts out}. 

Here, Apple does not have any explicit polarity clue in its context (see Algorithm~\ref{contextExtraction1}), though the sentiment expressed about it is negative. In this case, we take the value of NumNeg feature for Apple as $1$.
	% write about neutral comparative adjectives 

{\bf (b) Punctuation Marks:}
Using punctuations to express sentiment is a common practice in online social media. We look for the presence of two punctuation marks: question marks and exclamation marks in the context of an entity. We calculate two punctuation features for a comment: IsQuestion (presence or absence of a question mark), IsExclam (presence or absence of an exclamation mark)

%In online interactions, punctuation is commonly used to show the intensity of emotions. For example, {\em I like it!} and {\em I like it !!!!!!!!} are two different ways of writing the same text, but with different intensities of emotion. The intensity of positive emotion is higher in the latter case.  We extract question marks and exclamation marks from a comment and used their frequency of occurrence in the comment as features.

{\bf (c) Sentiment Strength:}
These features capture the strength of the sentiments expressed in comments. We used the SentiStrength algorithm~\cite{thelwall2012sentiment} to compute these features. The algorithm is specifically designed to calculate sentiment strength of short informal texts in online social media. For a piece of text, the algorithm computes two integral scores, one in the range of +1 (neutral) to +5 (highly positive) that is expressive of the positive sentiment strength of the text and other in the range -1 (neutral) to -5 (highly negative) for negative sentiment strength. A score of +1 and -1 for a text means that the text is neutral or has no sentiment. Using SentiStrength, we compute three features: PosStrength (positive sentiment strength score), NegStrength (negative sentiment strength score) and PosVsNegStrength (PosStrength/NegStrength).

{\bf (d) Comment-specific features:}
These features capture clues that are specific to news comments. %Comments often have sentiments embedded in sarcastic language. We observe that using rhetoric is one of the common ways of expressing sarcasm in comments. 
Users often use rhetorics in their comments to express negative sentiment about an entity. They begin their comments by writing rhetorical questions and/or asking rhetorical questions about entities. Rhetorical questions are questions that are not asked for the purpose of getting answers or information but rather to make a point effectively~\footnote{http://en.wikipedia.org/wiki/Rhetorical\_question}. Examples of rhetoric questions are {\em Where is my vote?}, {\em Can't you do anything right?} Let us consider the  following example comments:

{\bf Example 16:} {\em Why didn't} CBS {\em use the same guy to interview both} Obama {\em and} Romney{\em ?} Romney's {\em interview was tough and good. Can't say the same about} Obama's.  

{\bf Example 17:} {\em PLANS? What Plans?} Obama {\em has no plans for his second term.}

%1. {\em Why didn't CBS use the same guy to interview both Obama and Romney? Romney's interview was tough and good. Can't say the same about Obama's.}
%2. {\em PLANS? What Plans? Obama has no plans for his second term.}

These examples express implicit negative sentiment about CBS and Obama, respectively, without using explicit negative polarity clues. To capture these rhetorics, we design three binary features: IsFirstQues and IsEnQues. IsFirstQues checks whether the first sentence in the context of an entity is question or not. IsEnQues checks if an entity is present in a question sentence. To identify question sentences, we check for the presence of 5W1H and question marks in the sentence.

==> Files/confusionMatrix.tex <==
\begin{table}[htbp] 
\begin{centering}
%\small{
\begin{tabular}{@{}l c c @{}} 
\toprule
\multicolumn{2}{@{}l@{}}{\bf Classified As}&{\bf True Class} \\ 
\midrule
\multicolumn{3}{@{}l@{}}{\bf Unbalanced learning (F-1=$0.785$)}\\
\midrule
$+1$&$-1$& \\
\midrule
$2$&$20$&$+1$\\
$5$&$116$&$-1$\\
\midrule
\multicolumn{3}{@{}l@{}}{\bf Balanced learning (F-1=$0.596$)}\\
\midrule
$+1$&$-1$& \\
\midrule
$11$&$11$&$+1$\\
$56$&$65$&$-1$\\
\midrule
\multicolumn{3}{@{}l@{}}{\bf Balanced learning using ensembling, $n=2$ (F-1=$0.602$)}\\
\midrule
$+1$&$-1$& \\
\midrule
$13$&$9$&$+1$\\
$57$&$64$&$-1$\\
\bottomrule
\end{tabular} 
\caption{Classification performance in terms of confusion matrix and F-1 score of different classification models built on sentiment features. $n$ is the number of balanced samples used in the ensemble.}
%}
\label{resultClassification}  
\end {centering}
\end{table}

==> Files/contextTable.tex <==
\begin{table}[t]
\begin{centering}
%\begin{footnotesize}
%\begin{small}
%\begin{center}
	\begin{tabular}{@{} l p{2 in}@{}}
	%\begin{small}
	\toprule
	\textbf{Entity} & \textbf{Context}\\
	\midrule
	Democratic party&The of unrecognizable. The filthy democratic party with the CHICAGO POLITICAL THUG ATTITUDE NEEDS TO GO. Now. \\
	John F Kennedy& of is unrecognizable. Now.\\
	Republican& I'm PROUD to be a REPUBLICAN. Now.\\
	\bottomrule
	\end{tabular}
	\caption{Context extraction for Example 8.}
	\label{context}		
%end{small}
%\end{scriptsize}
\end{centering}
\end{table}

==> Files/dataTable.tex <==
\begin{table}[ht]
\begin{centering}
%\begin{footnotesize}
%\begin{small}
%\begin{center}
	\begin{tabular}{@{}l rl@{}}
	%\begin{small}
	\toprule
	%\textbf{Feature Name} & \textbf{Description}\\
	Total comments&$41,852,453$\\
	No. of conversations&$9,586,835$\\
	No. of reply comments&$21,830,249$\\
	No. of isolated comments&$10,435,369$\\
	%No. of users&$$\\
	\bottomrule
	\end{tabular}
	\caption{Data description.}
	\label{data}		
%end{small}
%\end{scriptsize}
\end{centering}
\end{table}

==> Files/entityTable.tex <==
\begin{table}[ht]
\begin{centering}
%\begin{footnotesize}
%\begin{small}
%\begin{center}
	\begin{tabular}{@{} l r@{}}
	%\begin{small}
	\toprule
	\textbf{Entity} & \textbf{Comment frequency}\\
	\midrule
	Barack Obama&$10,626,624$\\
	Mitt Romney& $4,658,983$\\
	Yahoo&$592,073$\\
	Google&$160,210$\\
	Microsoft&$21,680$\\
	Walmart&$80,256$\\
	Target&$108,578$\\
	\bottomrule
	\end{tabular}
	\caption{Document frequencies of some entities.}
	\label{entity}		
%end{small}
%\end{scriptsize}
\end{centering}
\end{table}


==> Files/featureRankPolarTable.tex <==
\begin{table}[ht]
\begin{centering}
	\begin{tabular}{@{} l @{}}
		\toprule
		Feature Name \\
		%All majority & 0.559&0.774&0.676\\
		NumNeg\\
		PosVsNeg\\
		NegStrnth \\
		IsQuesMark\\
		PosStrnth \\
		IsEnQues \\
		IsQuesFirst \\
		IsExclaim \\
		IsEnQuote \\
		NumPos \\
		PosVsNegStrnth \\
		\bottomrule
	\end{tabular}
	\caption{Feature ranking using Information gain.}
	\label{featureRank}
\end{centering}
\end{table}

==> Files/featureTable.tex <==
\begin{table*}[ht]
\begin{centering}
%\begin{footnotesize}
%\begin{small}
%\begin{center}
	\begin{tabular}{@{}l p{4.00 in}@{}}
	%\begin{small}
	\toprule
	\textbf{Feature Name} & \textbf{Description}\\
	\midrule
	\multicolumn{2}{@{}l@{}}{\textbf{Polarity clues}} \\
	\midrule
	NumPos & Number of postive polarity clues in entity's context.\\
	NumNeg & Number of negative polarity clues in entity's context.\\
	PosVsNeg & Number of positive polarity clue over negative polarity clue in the context. Calculated as (NumPos+1)/(NumNeg+1)\\
	\midrule
	\multicolumn{2}{@{}l@{}}{\textbf{Sentiment strength features}} \\
	\midrule
	PosStrength & Positive sentiment strength of the comment as given by SentiStrength algorithm.\\
	NegStrength & Negative sentiment strength of the comment as given by SentiStrength algorithm\\	
	PosVsNegStrength & PosStrength divided by NegStrength.\\		
	\midrule
	\multicolumn{2}{@{}l@{}}{\textbf{Punctuation Marks}} \\
	\midrule
	NumQues & Number of question marks in entity's context.\\
	IsQues & Whether the entity's context has a question mark or not (1 if yes, 0 otherwise)\\
	NumExclaim & Number of exclamation marks entity's context.\\ 
	IsExclaim & Whether the entity's context has an exclaimation mark or not (1 if yes, 0 otherwise)\\
	\midrule
	\multicolumn{2}{@{}l@{}}{\textbf{Comment-specific features}} \\
	\midrule
	IsFirstQues & Whether the first sentence in the entity's context is a question or not (1 if yes, 0 otherwise) \\
	IsEnQues & Whether the entity occur in a question sentence (1 if yes, 0 otherwise) \\
	IsEnQuote & Whether the entity occurs in a quoted phrase or not (1 if yes, 0 otherwise) \\
	%IsClueQuote & Whether a polarity clue occur in a quoted phrase or not (1 if yes, 0 otherwise)\\
	\bottomrule
	\end{tabular}
	%\end{footnotesize}
	%\end{small}
	\caption{Description of various features extracted from the context of an entity for polarity classification.}
	\label{features}		
%end{small}
%\end{scriptsize}
\end{centering}
\end{table*}

	%\midrule
	%\multicolumn{2}{@{}l@{}}{{\bf Domain-dependent features} (for a sentence containing 3 words $W_{i} ,W_{i+1}, W_{i+2}$ with POS tags $POS_{i}, POS_{i+1}, POS_{i+2}$ respectively.)} \\
	%\midrule
%	$BoW$&$W_{i} ,W_{i+1}, W_{i+2}$\\
	%$Uni+POS$&$W_{i}, POS_{i},  W_{i+1}, POS_{i+1},  W_{i+2},$ $POS_{i+2}$\\
	%$Uni+Bi$&$W_{i}, W_{i+1}, W_{i+1}, W_{i}W_{i+1},$ $ W_{i+1}W_{i+2}$\\
	%$Uni+Bi+POS$& $W_{i}, POS_{i},  W_{i+1}, POS_{i+1},  W_{i+2}, POS_{i+2},W_{i}W_{i+1}, W_{i}POS_{i+1},$ $POS_{i}W_{i+1}, W_{i+1}W_{i+2}, W_{i+1}POS_{i+2}, POS_{i+1}W_{i+2}$\\

==> Files/introductionOld.tex <==
\section{Introduction}
\label{intro}
Online news aggregator sites such as Yahoo News are a place for users to get in touch with recent developments across various domains. 
In addition to reading news articles, users post comments giving their opinions/sentiments about the entities discussed in the news articles, while interacting (agreeing or disagreeing) with other users. 
This has resulted in vast amounts of User Generated Content (UGC) in the form of user comments on these websites. 
Analyzing comments for opinions/sentiments of users is an interesting and challenging research problem. 
%In this work, we formulate the problem of sentiment analysis of user comments in Yahoo News, propose a methodology to automatically extract entities referred to in the comments and the user's sentiments towards them.

\comment{Research in sentiment analysis has been mainly focused in the domain of product reviews with recent works analyzing sentiments of social media content such as Twitter, Facebook, online forums, etc~\cite{sentiWords,ly2011product,sentiFacebook,Jiang2011}. Though there have been works on analyzing sentiments expressed in news articles~\cite{godbole2007large,devitt2007sentiment}, to the best of our knowledge, the problem of sentiment analysis of comments posted on news articles has not been addressed in the literature. We model the problem as a multi-class classification of sentiment into one of the three classes: positive, negative and neutral. We extract various features such as polarity clues, punctuations, content feautures and sentiment features for classification and experiment with different supervised machine learning algorithms.}
\vspace{0.2 cm}

%{\bf Why Sentiment Analysis of Comments on News Articles?}

Specifically, sentiment analysis of user comments posted on news articles can help understand the {\em user} better which, in turn, can be used to provide greater personalization and improve serving targeted ads to those users.
News sites cover a wide range of domains such as politics, sports, technology, and entertainment,  in contrast to other online social sites, including online forums (e.g., UbuntuForums for Ubuntu OS, and TripAdvisor for travel issues) and review sites (e.g., dpreview.com for digital cameras, and notebookreview.com for laptops), which are specific to a particular domain. Hence, the activity of a user in terms of posting comments is much more diverse in news sites as compared to other social platforms. 
%Also, a user associated with a news site is more likely to post comments on diverse topics. 

A comment on a news article usually contains sentiments of users about the entities in the article, although it is not uncommon for users to comment about unrelated entities they like or dislike. 
Analyzing sentiments of a particular user across domains (on various entities) will help obtain a {\em holistic} view of their personality\footnote{In adherence to Yahoo's privacy policy, all user activity is anonymized and the actual user's identity is unknown to us.}. 
For example, by looking at the sentiments of a user's comments on news articles related to politics, smartphones and online retail, her political orientation, preference for a particular mobile operating system (Android versus iOS) and liking for a particular online retailer (Walmart versus Ebay versus Target, etc.) may be inferred. 
Also, user sentiments across articles on a particular entity (e.g., Walmart or Obama) can be followed to see if and how the sentiment evolves. 
For example, a loyal user (for an entity) may turn into hostile or vice versa over a period of time (may or may not be due to certain actions of the entity), or a user may always remain loyal or hostile towards a particular entity. This information can be very helpful from marketting perspective. We pursue these research analyses as the part of our broader research goals. In the current work, we focus only on the problem of entity-specific sentiment analysis.

Analyzing sentiments of user comments on news articles has some interesting challenges, primarily the following: irrelevant entities and implicit sentiment.

{\bf Irrelevant entities:} Comments often have entities that are unimportant with respect to sentiment analysis. Let us consider the following examples:	

\vspace{1mm}
\noindent {\bf Example 1:} {\em Guess what?} Foxnews {\em poll:} Obama +9; CNN poll: Obama +7; Reuters/Ipsos poll: Obama +9. {\em I feel a landslide in the making. Gobama! Gobama! Gobama!}

\comment{
\vspace{1mm}
\noindent {\bf Example 2:} {\em This guy and} Chris Dodd {\em has ruined the economy when they in charged of} fannie mae {\em and} freddie mac.
}

\vspace{1mm}
\noindent {\bf Example 2:} Marci Alt {\em is an arsonist.} Google {\em her name and see the mugshot of this man like plaid wearing lesbian.}
\vspace{1mm}

	In the first example, the comment has positive sentiment about Obama, but the other entities (Foxnews, CNN, etc.) are unimportant from the point of view of sentiment analysis. 
	\comment{Similarly, in the second example, sentiment about Chris Dodd is negative and fannie mae and freddie mac are irrelevant for sentiment analysis.}
	In the second example, Marci Alt has negative sentiment and google does not have any sentiment. A named entity recognizer will identify all the entities in these examples which makes entity-specific sentiment analysis difficult in these cases. This is {\em different} from sentiment analysis of reviews, where targets of sentiment (generally a product and its features) are known. 
	To address this challenge, we model it as a binary classification problem of classifying entities into neutral and polar classes. Irrelevant entities are identified as neutral entities, i.e., entities about which no sentiment is expressed in the comment. We {\em propose} the use of features that are specific to entities such as whether an entity is of person type or not and their grammatical role in comments (whether an entity is a subject, direct object or prepositional object).
	
{\bf Implicit sentiment}: Users often express sentiments implicitly in their comments by using ironies, analogies, rhetorics, making very less use of emoticons~\footnote{We observe that unlike other social media data, comments in news articles make very less use of important sentiment clues such as emoticons. Emoticons have been extensively used in detecting sentiments of informal texts on social media~\cite{ASONAM, feelBetter}, etc.}, which makes it hard to detect their sentiment~\cite{gonzalez2011identifying,utsumi2000verbal}. Let us consider the following examples. 
		
\vspace{1mm}
\noindent {\bf Example 3:} {\em I've heard that} Hillary Clinton {\em modeled herself after Nurse Ratched}.
	
\vspace{1mm}	
\noindent {\bf Example 4:} {\em Who on earth would even buy} Facebook {\em stock?}

\vspace{1mm}
		The first example has a negative sentiment about Hillary Clinton because it compares her with ``Nurse Ratched''\footnote{Nurse Ratched is a negative fictional character}. The second example is a rhetorical question expressing a negative sentiment about Facebook. A typical sentiment classifier will label these examples as neutral\footnote{SentiStrength (a state-of-the-art sentiment analysis tool) labels these instances as neutral.} as there are no sentiment clues present in them. To address this challenge, we use two comments-specific features in our polarity classification model, which capture sentiments expressed through rhetorical questions. We check if a comment starts with a question and if a comment contains entities in a question sentence.


{\bf Contributions:} Our work makes the following contributions:
\begin{itemize}
	\item We propose a study of entity-specific sentiment analysis of news comments. To the best of our knowledge, there are no reported works on this problem so far. Although there have been works on analyzing sentiments of news articles, the current problem is significantly different (as detailed in Section 2).
	\item We found that for entity-specific sentiment analysis of news comments a difficult task is to segment comments into contexts of multiple entities across domains. We design and evaluate an algorithm for context extraction of entities.
	\item We propose two novel non-lexical features for neutral-polar classification: IsPerson and IsSubjObj. We show that these features are more informative than the lexicon-based features and bag-of-words that are used in previous works on subjectivity classification.  For polarity classification of entities, we use two novel comment-specific features and show that adding these features improves the polarity classification performance. These features have not been used in sentiment classification.
	\end{itemize}

The rest of the paper is organized as follows. The next section reviews relevant literature of sentiment analysis. Section~\ref{approach} formulates the problem and describes features used for sentiment classification. Section~\ref{experiments} gives details about the data, evaluates the proposed approach and discusses experimental results. Section~\ref{sec:Conclusion} concludes the paper.



==> Files/introductionOld1.tex <==
\section{Introduction}
\label{intro}
Online news aggregator sites such as Yahoo News are a place for users to get in touch with recent developments across various domains. 
In addition to reading news articles, users post comments giving their opinions/sentiments about the entities discussed in the news articles, while interacting (agreeing or disagreeing) with other users. 
This has resulted in vast amounts of User Generated Content in the form of user comments on these websites. 
Analyzing comments for opinions/sentiments of users is an important problem. %interesting and challenging research problem. 
%In this work, we formulate the problem of sentiment analysis of user comments in Yahoo News, propose a methodology to automatically extract entities referred to in the comments and the user's sentiments towards them.
%\comment{Research in sentiment analysis has been mainly focused in the domain of product reviews with recent works analyzing sentiments of social media content such as Twitter, Facebook, online forums, etc~\cite{sentiWords,ly2011product,sentiFacebook,Jiang2011}. Though there have been works on analyzing sentiments expressed in news articles~\cite{godbole2007large,devitt2007sentiment}, to the best of our knowledge, the problem of sentiment analysis of comments posted on news articles has not been addressed in the literature. We model the problem as a multi-class classification of sentiment into one of the three classes: positive, negative and neutral. We extract various features such as polarity clues, punctuations, content feautures and sentiment features for classification and experiment with different supervised machine learning algorithms.}
%\vspace{0.2 cm}
%{\bf Why Sentiment Analysis of Comments on News Articles?}
Specifically, sentiment analysis of user comments posted on news articles can help understand the {\em user} better which, in turn, can be used to provide greater personalization and improve serving targeted ads to those users.
News sites cover a wide range of domains such as politics, sports, technology, and entertainment,  in contrast to other online social sites, including online forums (e.g., UbuntuForums and TripAdvisor) and review sites (e.g., dpreview.com for digital cameras and notebookreview.com for laptops), which are specific to a particular domain. Hence, the activity of a user in terms of posting comments is potentially much more diverse in news sites as compared to other social platforms. 
%Also, a user associated with a news site is more likely to post comments on diverse topics. 

Comments on a news article usually contain sentiments of users about the entities in the article, although it is not uncommon for users to comment on unrelated entities that they like or dislike. 
Analyzing sentiments of a particular user across domains (on various entities) can help obtain a {\em holistic} view of their personality\footnote{In adherence to Yahoo's privacy policy, all user activity is anonymized and the actual user's identity is unknown to us.}. 
For example, the sentiments of a user's comments on news articles related to politics, smartphones and online retail may help infer her political orientation, preference for a particular mobile operating system (Android vs. iOS) and liking of a particular online retailer (Walmart vs. Target). 
User sentiments across articles on an entity (e.g., iPhone) can be followed to determine how sentiments evolve or change over time. 
%For example, a loyal user (for an entity) may turn into hostile or vice versa over a period of time (may or may not be due to certain actions of the entity), or a user may always remain loyal or hostile towards a particular entity. 
This information can be very helpful from a marketing perspective. %We pursue these research analyses as the part of our broader research goals. In the current work, we focus only on the problem of entity-specific sentiment analysis.

However, despite the evidence of strong value for identifying sentiments of user comments on news articles, the problem remains inherently difficult due to several main challenges: irrelevant entities and implicit sentiment.

{\bf Irrelevant entities:} Comments often have entities that are not important with respect to sentiment analysis. Let us consider the following examples:	

\vspace{1mm}
\noindent {\bf Example 1:} {\em Guess what?} Foxnews {\em poll:} Obama +9; CNN poll: Obama +7; Reuters/Ipsos poll: Obama +9. {\em I feel a landslide in the making. Gobama! Gobama! Gobama!}

\comment{
\vspace{1mm}
\noindent {\bf Example 2:} {\em This guy and} Chris Dodd {\em has ruined the economy when they in charged of} fannie mae {\em and} freddie mac.
}

\vspace{1mm}
\noindent {\bf Example 2:} Marci Alt {\em is an arsonist.} Google {\em her name and see the mugshot of this man like plaid wearing lesbian.}
\vspace{1mm}

In the first example, the comment has positive sentiment about Obama, but the other entities (Foxnews, CNN, etc.) are not important from the point of view of sentiment analysis. 
\comment{Similarly, in the second example, sentiment about Chris Dodd is negative and fannie mae and freddie mac are irrelevant for sentiment analysis.}
In the second example, Marci Alt has negative sentiment and Google does not have any sentiment. {\color{red}A named entity recognizer will identify all the entities in these examples which makes entity-specific sentiment analysis difficult in these cases.} This is {\em different} from sentiment analysis of reviews, where targets of sentiment (generally a product and its features) are known. 
%To address this challenge, we model it as a binary classification problem of classifying entities into neutral and polar classes. Irrelevant entities are identified as neutral entities, i.e., entities about which no sentiment is expressed in the comment. We {\em propose} the use of features that are specific to entities such as whether an entity is of person type or not and their grammatical role in comments (whether an entity is a subject, direct object or prepositional object).
	
{\bf Implicit sentiment}: Users often express sentiments implicitly in their comments by using ironies, analogies, rhetorics, making very less use of emoticons~\footnote{We observe that unlike other social media data, comments in news articles make very less use of important sentiment clues such as emoticons. Emoticons have been extensively used in detecting sentiments of informal texts on social media~\cite{ASONAM, feelBetter}, etc.}, which makes it hard to detect their sentiment~\cite{gonzalez2011identifying,utsumi2000verbal}. Let us consider the following examples. 
		
\vspace{1mm}
\noindent {\bf Example 3:} {\em I've heard that} Hillary Clinton {\em modeled herself after Nurse Ratched}.
	
\vspace{1mm}	
\noindent {\bf Example 4:} {\em Who on earth would even buy} Facebook {\em stock?}

\vspace{1mm}
		The first example has a negative sentiment about Hillary Clinton because it compares her with ``Nurse Ratched''\footnote{Nurse Ratched is a negative fictional character}. The second example is a rhetorical question expressing a negative sentiment about Facebook. A typical sentiment classifier will label these examples as neutral\footnote{SentiStrength (a state-of-the-art sentiment analysis tool) labels these instances as neutral.} as there are no sentiment clues present in them. %To address this challenge, we use two comments-specific features in our polarity classification model, which capture sentiments expressed through rhetorical questions. We check if a comment starts with a question and if a comment contains entities in a question sentence.


{\bf Contributions:} Our work makes the following contributions:
\begin{itemize}
	\item We propose a study of entity-specific sentiment analysis of news comments. To the best of our knowledge, there are no reported works on this problem so far. Although there have been works on analyzing sentiments of news articles, the current problem is significantly different (as detailed in Section 2).
	\item We found that for entity-specific sentiment analysis of news comments a difficult task is to segment comments into contexts of multiple entities across domains. We design and evaluate an algorithm for context extraction of entities.
	\item We propose two novel non-lexical features for neutral-polar classification: IsPerson and IsSubjObj. We show that these features are more informative than the lexicon-based features and bag-of-words that are used in previous works on subjectivity classification.  For polarity classification of entities, we use two novel comment-specific features and show that adding these features improves the polarity classification performance. These features have not been used in sentiment classification.
	\end{itemize}
	
Although in this paper we focus on the design of accurate approaches to identifying entity-based sentiment analysis of user comments in online news sites, our objective is to integrate this classification component in the context of opinion mining to improve ad targeting/effective advertising, content personalization and political campaign planning.

The rest of the paper is organized as follows. The next section reviews relevant literature of sentiment analysis. Section~\ref{approach} formulates the problem and describes features used for sentiment classification. Section~\ref{experiments} gives details about the data, evaluates the proposed approach and discusses experimental results. Section~\ref{sec:Conclusion} concludes the paper.



==> Files/resultContextNeutralTable.tex <==
\begin{table}[th]
\begin{centering}
	\begin{tabular}{@{} p{1.6 in} c c c @{}}
		\toprule
		{\bf Model}&{\bf Pr.}&{\bf Re.}&{\bf F-1} \\
		\midrule
		\multicolumn{4}{c}{{\bf Neutral-polar Classification}} \\
		\midrule
		Baseline & $0.646$ & $0.645$ & $0.645$ \\	
		{\bf Proposed model}&  ${\bf 0.654}$ &  ${\bf 0.654}$&  ${\bf 0.654}$  \\	
		\midrule
		\multicolumn{4}{c}{{\bf Positive-negative Classification}} \\
		\midrule
		Baseline &$0.472$ & $0.492$& $0.491$\\
		{\bf Proposed model} & ${\bf0.56}$ & ${\bf0.569}$ & ${\bf0.542}$\\	
		\bottomrule
	\end{tabular}
	\caption{Effects of the context-extraction algorithm on neutral-polar and positive-negative classification.}
	\label{contextResults}
\end{centering}
\end{table}

==> Files/resultContextPolarTable.tex <==
\begin{table}[ht]
\begin{centering}
	\begin{tabular}{@{} p{1.6 in} c c c @{}}
		\toprule
		{\bf Model}&{\bf Precsion}&{\bf Recall}&{\bf F-1} \\
		\midrule
		-Coreference &0.515 & 0.420& 0.463\\
		-localContext & $0.527$ & $0.502$ & $0.466$\\	
		-coreference-LocalContext & $0.506$ & $0.510$ & $0.507$ \\	
		Proposed model& $0.553$ & $0.557$ & $0.553$  \\	
		\bottomrule
	\end{tabular}
	\caption{Effects of different coreference resolution and local context extraction on neutral-polar classification..}
	\label{contextPolarResults}
\end{centering}
\end{table}
